SGX-SSD: A Policy-based Versioning SSD with Intel SGX

This paper demonstrates that SSDs, which perform device-level versioning, can be exposed to data tampering attacks when the retention time of data is less than the malware's dwell time. To deal with that threat, we propose SGX-SSD, a SGX-based versioning SSD which selectively preserves file history based on the given policy. The proposed system adopts Intel SGX to implement the version policy management system that is safe from high-privileged malware. Based on the policy, only the necessary data is selectively preserved in SSD that prevents files with less priority from wasting space and also ensures the integrity of important files.

==> related.tex <==
\section{Related Work}
\label{sec:related}
\vspace{-0.1in}

%기존 백업 소프트웨어는 (1)local 저장소; (2)network attached remote 저장소; (3)cloud storage(ex: Dropbox, Google Cloud)에 백업을 수행한다.
%(1), (2)는 권한을 향상한 랜섬웨어의 주요 공격 대상이다~\cite{ryuk1,ryuk2,ransomware_many}. 
%(3)는 클라이언트 단의 랜섬웨어로부터 백업 데이터를 보호할 수 있지만, 
%\textcolor{green}{4.2섹션 내용이 추가되어 공간이 없으면 이 내용은 날려도 됩니다. 크게 중요하지 않고 이미 intro에서 언급니 되었습니다.}
%대규모 네트워크 연결 서버로 인한 TCB의 크기가 {\sgxssd}보다 훨씬 커서 취약점이 생기면 대규모의 데이터 손실이 발생할 수 있다. 
%이 문제를 해결하기 위해, 

% 최근에 작은 TCB를 제공하는 SSD 레벨의 데이터 보호 시스템으로는 (1)탐지 기반 SSD~\cite{amoeba,SSDinsider,flashguard,ransomblocker};(2)상태 보존 SSD(Almanac)이 있다. 
% 하지만, 지능적인 멀웨어는 기존과는 다른 패턴으로 데이터를 변조하여 (1)의 탐지 시스템을 우회할 수 있다. 
% (2)는 모든 백업 데이터에 똑같이 적용되는 짧은 RT가 스토리지 전체를 vulnerable하게 만든다. 

% Pesos~\cite{pesos}는 access control기반의 스토리지로 {\sgxssd}보다 풍부한 policy를 제공한다.
% 하지만, Pesos의 보안 scope은 원격 서버에 제한하고, 클라이언트 시스템은 신뢰한다고 가정하기 떄문에, 클라이언트 머신에 멀웨어가 침입하면 데이터를 보호할 수 없다.

% Inuksuk~\cite{inuksuk}은 intel TXT와 self-encryption disk(SED)를 활용하여 데이터를 protected partition으로 복사하여 보호한다. 
% Inuksuk은 {\sgxssd}와 마찬가지로 선별적으로 파일을 디스크에서 보호할 수 있다.
% 하지만, Inuksuk은 protected partition으로 데이터를 백업하는 오버헤드가 매우 클 뿐 아니라(ex: 85.6MB의 파일을 백업하는데 23.38초 소모~\cite{inuksuk}), 데이터가 백업하는 동안에는 시스템이 중단되어 서비스가 멈춰버리는 문제가 있다. 
% 긴 시간의 시스템 중단 문제 때문에, Inuksuk은 데이터의 실시간 백업이 불가능하고, 백업할 파일의 크기와 백업 주기가 그만큼 제한된다.
% 특히, 서비스 중단이 매우 민감한 문제를 낳는 client-server 모델에서는 서비스 중단을 막기 위해서는 inuksuk서버를 추가적으로 배치해야 한다. 
% 반면 {\sgxssd}는 호스트 서비스와 {\texttt{PV-SSD}}의 버저닝이 동시에 수행될 뿐 아니라, 버저닝으로 유발되는 오버헤드가 매우 적다.


Recent SSD-level data protection systems that provide a small TCB include (i) detection-based SSD~\cite{amoeba,SSDinsider,flashguard,ransomblocker} and (ii) state-preserving SSD (Project Almanac).
However, the intelligent malware can bypass the detection system of (i) by modulating the data in a pattern different from the known ones.
(ii) makes the entire storage vulnerable since the short RT is applied to all data equally.
Pesos~\cite{pesos} is the access-control-based object storage and provides richer policy than {\sgxssd}.
However, the security scope of Pesos is limited to remote servers, and assumes that the client system is trusted. Therefore, data cannot be protected when malware enters the client machine.

Inuksuk~\cite{inuksuk} uses Intel TXT and self-encryption disk (SED) to protect data by copying it to a protected partition.
Inuksuk, like {\sgxssd}, can selectively protect files in the disk.
However, Inuksuk has a very large overhead of backing up data to a protected partition (e.g. 23.38 seconds to back up 85.6MB of JPG files~\cite{inuksuk}), and the whole system is interrupted while data is being backed up.
Due to the long system downtime problem, Inuksuk is unable to back up data in real time, and the size of the files to be backed up and the backup cycle is limited.
In particular, in the client-server model, where service interruption is very sensitive, an Inuksuk server must be additionally deployed to prevent service interruption.
On the other hand, {\sgxssd} not only performs host service and {\texttt{PV-SSD}}'s versioning at the same time, but also has very little overhead caused by versioning.
%On the other hand, {\sgxssd} not only performs versioning of the host service and {\texttt {PV-SSD}} at the same time, but also has very little overhead caused by versioning.
